TPA3D: Triplane Attention for Fast Text-to-3D Generation

Due to the lack of large-scale text-3D correspondence data, recent text-to-3D generation works mainly rely on utilizing 2D diffusion models for synthesizing 3D data. Since diffusion-based methods typically require significant optimization time for both training and inference, the use of GAN-based models would still be desirable for fast 3D generation. In this work, we propose Triplane Attention for text-guided 3D generation (TPA3D), an end-to-end trainable GAN-based deep learning model for fast text-to-3D generation. With only 3D shape data and their rendered 2D images observed during training, our TPA3D is designed to retrieve detailed visual descriptions for synthesizing the corresponding 3D mesh data. This is achieved by the proposed attention mechanisms on the extracted sentence and word-level text features. In our experiments, we show that TPA3D generates high-quality 3D textured shapes aligned with fine-grained descriptions, while impressive computation efficiency can be observed.

==> table/clip_r_precision.tex <==
\begin{table}[t]
    \centering
    \caption{\ben{\textbf{Evaluation of text-shape alignment in terms of CLIP R-Precision@5 ($\uparrow$)}. Compared to TAPS3D taking only sentence-level features into consideration, our TPA3D performs additional word-level refinement and results in improved alignment between the generated shape and the given text prompts.}}
    \resizebox{0.8\textwidth}{!}{
        {\renewcommand{\arraystretch}{1.3}
        \begin{tabular}{l|ccc|cc}
            \toprule
            \multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{ShapeNet} & \multicolumn{2}{c}{OmniObject3D} \\
            \cline{2-6}
            \multicolumn{1}{l|}{} & Car & Chair & Motorbike & Vehicle & Accessory \\ \midrule
            TAPS3D~\cite{wei2023taps3d} & 12.55 & 7.52 & 5.00 & 9.47 & 6.67 \\
            Ours (TPA3D) & \textbf{80.94} & \textbf{38.58} & \textbf{24.76} & \textbf{65.26} & \textbf{64.44} \\
            \bottomrule
        \end{tabular}}}
    \label{table:clip_r_precision}
\end{table}

==> table/fid.tex <==
\begin{table}[t]
\centering
\caption{\ben{\textbf{Visual quality comparisons in terms of FID ($\downarrow$).} Note that GET3D is an unconditional 3D generator, with performances serving as upper bounds for ShapeNet~\cite{chang2015shapenet}. And, TAPS3D is only conditioned on sentence-level features for text-guided 3D generation.}}
\resizebox{0.8\textwidth}{!}{
    {\renewcommand{\arraystretch}{1.25}
    \begin{tabular}{l|ccc|cc}
    \toprule
    \multicolumn{1}{l|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{ShapeNet} & \multicolumn{2}{c}{OmniObject3D} \\
    \cline{2-6}
    \multicolumn{1}{l|}{} & \hspace{7mm}Car\hspace{7mm} & \hspace{4mm}Chair\hspace{4mm} & \hspace{2mm}Motorbike\hspace{2mm} & \hspace{1mm}Vehicle\hspace{1mm} & \hspace{3mm}Accessory\hspace{3mm} \\ \midrule \midrule
    GET3D~\cite{gao2022get3d} & \textbf{11.50} & \textbf{22.75} & \textbf{49.98} & \underline{98.15} & \underline{145.66} \\
    \midrule
    TAPS3D~\cite{wei2023taps3d} & 26.37 & 44.70 & 84.83 & 152.34 & 172.14 \\
    Ours (TPA3D) & \underline{18.50} & \underline{38.11} & \underline{77.69} & \textbf{68.80} & \textbf{83.31} \\
    \bottomrule
    \end{tabular}}
}
\label{table:fid}
\end{table}

==> table/quantitative.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Quantitative results in terms of FID ($\downarrow$) and CLIP R-Precision@5 ($\uparrow$).} Compared to TAPS3D taking only sentence-level features into consideration, our TPA3D performs additional word-level refinement and results in better visual quality and improved alignment between the generated shape and the given text prompts. Note that GET3D is an unconditional 3D generator, with performances serving as upper bounds. }
\resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccc}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{FID $\downarrow$} & \multicolumn{3}{c}{CLIP-R Precision $\uparrow$} \\ 
        \cline{2-7}
        \multicolumn{1}{l|}{} & \hspace{4mm}Car\hspace{4mm} & \hspace{2mm}Chair\hspace{2mm} & Motorbike & Car & Chair & Motorbike \\
        \midrule \midrule
        GET3D~\cite{gao2022get3d} & 11.50 & 22.75 & 49.98 & - & - & - \\
        \midrule
        TAPS3D~\cite{wei2023taps3d} & 26.37 & 44.70 & 84.83 & {12.55 $\pm$ 3.00} & {7.52 $\pm$ 1.95} & {5.00 $\pm$ 5.00} \\
        Ours (TPA3D) & 18.50 & 38.11 & 77.69 & \textbf{80.94 $\pm$ 2.99} & \textbf{38.58 $\pm$ 2.28} & \textbf{24.76 $\pm$ 4.67} \\
        \bottomrule
    \end{tabular}
}
\label{table:quantitative}
\end{table}
